Putting a Padlock on Lambda -- Integrating vTPMs into AWS Firecracker

When software services use cloud providers to run their workloads, they place implicit trust in the cloud provider, without an explicit trust relationship. One way to achieve such explicit trust in a computer system is to use a hardware Trusted Platform Module (TPM), a coprocessor for trusted computing. However, in the case of managed platform-as-a-service (PaaS) offerings, there is currently no cloud provider that exposes TPM capabilities. In this paper, we improve trust by integrating a virtual TPM device into the Firecracker hypervisor, originally developed by Amazon Web Services. In addition to this, multiple performance tests along with an attack surface analysis are performed to evaluate the impact of the changes introduced. We discuss the results and conclude that the slight performance decrease and attack surface increase are acceptable trade-offs in order to enable trusted computing in PaaS offerings.

==> content/conclusion.tex <==
\section{Conclusion}\label{conclusion}
% \todo[inline]{Add the mention that you contacted Firecrackers maintainers for real-life impact :)}
This project has integrated software TPM support into the Firecracker VMM~\footnote{The maintainers of Firecracker have been contacted through GitHub Issues, see \url{https://github.com/firecracker-microvm/firecracker/issues/3629}.} along with measuring the performance and security impact of the additions.
%Taking into account the current support for virtio devices in Firecracker and taking inspiration from similar VMM projects, the modifications made to Firecracker resulted in a mere 2\% increase in lines of code.
By incorporating the TPM support, the memory overhead of the Firecracker process saw a negligible increase.
When including the vTPM process in the memory overhead, the memory overhead increased significantly. 
Nevertheless, the overhead remains a small percentage of the total memory allocated to a VM, and would, if used in practice, remain an opt-in feature for customers. 

The startup time increased significantly when TPMs were allocated on demand; however, when using a resource pool with pre-allocated vTPMs, the startup times were kept at an acceptable level.
Yet, there is still potential to further improve these metrics even further by adjusting the resource pool algorithm based on the workload and the specific hardware used.

Regarding the attack surface, there is an increase originating from the extended communication between the VM and external processes. 
However, considering that other virtio devices are already supported, the extended support for a virtio TPM fits into the Firecracker device model and does not extend the attack surface there. 
Therefore, the additional attack vector lies in the actual TPM implementation, which could easily be interchanged and hardened to mitigate security concerns.

In conclusion, the incorporation of a software TPM into the Firecracker VMM does not have a significant performance decrease. 
Instead, the extended use case, which features additional trust capabilities and assurance, compensates for the slight deterioration in performance.


==> content/future_work.tex <==
\section{Future Work}
As this work is aimed at a specific building block that enables trusted computing for PaaS offerings, there are several improvement areas and subfields that would benefit from future research. 

\subsection{VM Exits}
One metric that is neither evaluated nor analysed is the number of \emph{VM exits} occurring.
A VM exit is when control is transferred from execution within the VM to the hypervisor code, commonly occurring when a VM interacts with an emulated device. 
As VM exits can be considered an attack vector~\cite{szefer_eliminating_2011}, it would therefore be beneficial to compare the number of VM exits with and without a TPM.
VM exits require significant insight into KVM components to be able to analyse the different reasons behind the exits. 
Hence, the topic of VM exits have not been researched in this work as it deviates from the main purpose of this work.

\subsection{vTPM Trust Establishment at Scale}
%As mentioned in \autoref{practical_application}, future research and work is also needed to apply the results of this work in practice. 
Within practical applications, there is also multiple research subfields to be further worked upon.
One such area is trust processes and trust relationships, related to simulated TPM manufacturing and remote attestation. 
The concepts described in this project need to be adapted to a larger scale to be applicable for CSPs in practice. 

\subsection{Trusted Late Launch}
%Another subfield lies within OS support for trusted execution of workloads, where further research is needed to apply it to PaaS offerings.
%This work only uses Linux; however, other types of operating systems, such as unikernels similar to OSv could be more applicable. 
%An issue with OSv taking trusted computing into account is that there is no integrity measurement system or TPM support, which is a topic that would benefit from continued research. 
Efforts can also be made to implement trusted late launch functionality, where a VM can boot before it is known what workload it will execute, to later receive the workload and perform integrity measurements. 
By using a late launch, the startup time for workloads would be able to be reduced even further. 
%Alongside late launch capabilities, more work can be done on improvements to the Linux kernel boot time, as lower boot times would benefit a CSP regardless of whether late launch is used or not.

Further testing could also be beneficial to optimise the process and overhead from starting and using a vTPM in Firecracker.
Similar to how \textcite{manco2017my} examine the overhead of short-lived lightweight VMs whilst keeping isolation properties, it would be interesting to see what impact the vTPM support can have on more applied use cases.
However, optimising the startup time would require knowledge of the vendor specific resources and the Firecracker VMM.


%\subsection{Protection Against Memory Leaks}
\subsection{Alternative vTPM Implementation}
The vTPM implementation used is important with regard to the security of a trusted PaaS offering by a CSP. 
As mentioned in \autoref{disc_security_evaluation}, multiple actions can be taken to further isolate a Linux process to mitigate potential vulnerabilities. 
One potential research topic is to implement a vTPM in a memory-safe language, effectively protecting it against memory corruption attacks similar to those seen previously with vTPMs~\cite{mitre_corporation_cve_2023}.

\subsection{Migrations of VMs}
Another relevant research avenue is snapshots and migrations of VMs. 
Although previous work has been conducted with other VMMs regarding this topic~\cite{vtpm-vm-migration}, it falls outside the scope of this thesis and can be considered as potential future work.




==> content_new/benchmark_results.tex <==
\section{Benchmark and Results}\label{bench_resul}
%In order to answer our research questions, we describe how our performance tests operate and present the results of these tests in this section.
%We also analyse the changes in the attack surface.
To address our research questions, this section describes our performance tests, presents the results, and analyses changes in the attack surface.

\subsection{Design of the Test Suite}
\label{perftest-hardware}
%The performance tests are performed using CloudLab, which is a scientific infrastructure that gives bare metal access to cloud computing resources~\cite{duplyakin_design_cloudlab_2019}.  
%More specifically, the tests run on an instance consisting of two Intel Xeon Gold 6142 with 16 cores each and 384 GB of memory.
We conducted performance tests on CloudLab, a scientific infrastructure providing bare metal access to cloud computing resources~\cite{duplyakin_design_cloudlab_2019},
using two Intel Xeon Gold 6142 CPUs with 16 cores each and 384 GB of memory. 

\label{method-perf-test-suite}
%The performance test suite runs multiple scenarios with multiple setups. 
%The first setup, \emph{baseline} runs an unmodified Firecracker binary without a TPM, to serve as a comparison value. 
%The second setup, \emph{on demand} runs the modified Firecracker binary and provisions keys and starts a vTPM right before each VM is started.
%The third setup, \emph{pool} maintains a resource pool of already provisioned vTPMs and allocates one of them to each Firecracker VM before starting the VM. 
Three setups were tested: \emph{baseline} (unmodified Firecracker, to serve as a comparison value), \emph{on demand} (modified Firecracker that starts a vTPM right before each VM), and \emph{pool} (using a pre allocated resource pool of vTPMs). 

%Regarding the VM OS used, a Linux kernel compiled with a virtio-tpm driver along with a simple init script is used.
%The init script also shuts down the VM directly.
%The reason to not start any actual service is to minimise the number of components that can impact the startup time.
%The same OS configuration is used for all startup time tests. 
A Linux OS with a virtio-tpm driver was used with along with a simple init script that also handles VM shutdown.
To minimise the impact on startup time, additional services were not started. 
This OS configuration was consistent for all startup time tests.

The scenarios executed are the following:
\begin{itemize}
    \item 500 VMs, serially executed
    \item 1000 VMs, 50 running concurrently
\end{itemize}
These scenarios are the same as those used in benchmarks made comparing Firecracker with QEMU and Cloud-Hypervisor~\cite{firecracker-paper}.

Memory overhead of adding TPMs to VMs was also measured, with different VM sizes for stability. 
This assesses VM memory usage, disregarding available memory inside the VM. 
We used the \emph{pmap}~\cite{cahalan_pmap1_nodate} tool to measure non-shared memory, indicating scalability. 
Linux shares physical memory for processes with the same read-only memory, making it insignificant in systems with thousands of VMs.
%In addition to the startup time metric, we also measured the memory overhead of adding the TPM to the VM.
%The memory overhead describes the memory usage of each VM, disregarding the memory actually available inside the VM. 
%However, different VM memory sizes were used to verify that the memory overhead was stable.
%Memory overhead is measured using the \emph{pmap}~\cite{cahalan_pmap1_nodate} tool, which displays Linux process memory maps.
%Only non-shared memory is counted, as it represents how the system scales with more VMs.
%Linux allocates the same physical memory region for processes using the same read-only memory, therefore, it does not have an impact on a system with thousands of VMs. 
The memory evaluates the 3 setups: baseline, modified excluding vTPM memory, and modified including vTPM memory.

%The memory of the TPM pool is not considered, as it is not part of either the Firecracker process or the vTPM process. 
%In a real-world scenario, the pool itself would be implemented by the cloud provider to optimise for their use case. 
We excluded TPM pool memory since it doesn't impact Firecracker or vTPM processes. 
In a real-world scenario, the pool would be also be implemented by and optimised for the cloud provider. 

\subsection{Pooling Algorithm}
\label{pooling_algorithm}
%For the case of running VMs with TPMs allocated from a pool, the pool adheres to a specific resource pooling algorithm. 
%The purpose of using a pool is to move the resource allocation time from a critical point in time to a time where resources and time are less scarce. 
%A characteristic of a vTPM resource is that it can be used by only one VM throughout its lifecycle, which becomes a strict requirement of the resource pool. 
%The algorithm implemented for this project is a simple pre-allocated buffer, where vTPMs are provisioned and started when the pool is created.
In the case of VMs using TPMs from a pool, we follow a specific resource pooling algorithm. 
The goal is to allocate resources at a less critical time. 
A vTPM can only be used by one VM during its lifecycle, a strict requirement for the pool. 
We implemented a simple pre-allocated buffer to allocate TPMs.

\subsection{Results}
This chapter presents the test results, mainly the effects of integrating TPMs into Firecracker with regard to performance and security. 
%Based on these scenarios, the results are visualised using a graphed \textit{cumulative distribution function} (CDF) of the startup times along with a table that shows a numerical interpretation of the samples.
%To ensure that no measurement errors occurred, the startup time measured from the performance tests was compared with the time reported from the internal boot timer device in the Firecracker hypervisor. 
%The difference between the two was of reasonable size, ranging from $10-20$\%, implying no noteworthy errors.
We use \textit{cumulative distribution function} (CDFs) and tables to visualise and analyse the results.
To validate accuracy, we compared the startup time measured during performance tests with the time reported by Firecracker's internal boot timer device. 
The difference, approximately $10-20$\%, indicates negligible measurement errors.

\subsubsection*{Startup time scenario 1, 500 VMs, no concurrency}
The results of the scenario when running 500 VMs can be seen as a chart of the CDF in \autoref{fig:boottime_chart_500} and as numerical data in \autoref{tab:boottime_table_500}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=80mm]{figure/boottime_chart_500.pdf}
    \caption[Distribution of Boot Times for 500 VMs]{Boot time for 500 VMs serially executed}
    \label{fig:boottime_chart_500}
\end{figure}
\begin{table}[h]
    \centering
\csvreader[
  tabular=lrrrrrr,
  table head=\toprule {Type} & {p95} & {p95 Change} & {Std. Deviation} \\\midrule,
  late after last line=\\\bottomrule\newline
]{
  figure/boottime_table_500.csv
}{}{\csvcoli & \csvcolv & \csvcolvi & \csvcolvii}
\caption[Boot Times for 500 VMs]{Boot time for 500 VMs serially executed}
\label{tab:boottime_table_500}
\end{table}

An important aspect is the standard deviation that demonstrates the width of each CDF.
As can be seen in \autoref{tab:boottime_table_500}, the difference between the baseline and the pool implementation is significantly smaller in comparison to the difference between the baseline and the on demand implementation. 
%With regard to absolute numbers, the p95 column, showing the 95th percentile, tells us that the same pattern is seen here. 
%In general, the pool implementation performs slightly worse than the baseline; however, if the TPMs are allocated on demand, the results display a significantly worse boot time.
Reviewing the p95 (95th percentile) column, we see a similar trend. 
In general, the pool implementation performs slightly worse than the baseline. 
However,  on-demand TPM allocation results in significantly worse boot times.

\subsubsection*{Startup time scenario 2, 1000 VMs, 50 concurrent VMs}
Considering the other scenario, with 1000 VMs in total and 50 of them running concurrently, as can be seen in \autoref{fig:boottime_chart_1000} and \autoref{tab:boottime_table_1000}, the result changes. 
%The similarity regarding the CDF of the baseline and the pool setup is less apparent, and the CDF for the pool setup is slightly wider. 
%However, the pool setup still performs significantly better in comparison to the on demand setup.
%A major overall is that the deviations of all three setups increase by at least three times from scenario 1. 
The CDF similarity between the baseline and pool setups is less apparent, with a slightly wider pool setup CDF. 
However, the pool setup still outperforms the on-demand setup significantly. 
Overall, the deviations in all three setups increase by at least three times from scenario 1.

\begin{figure}[h]
    \centering
    \includegraphics[width=80mm]{figure/boottime_chart_1000.pdf}
    \caption[Distribution of Boot Times for 1000 VMs]{Boot time for 1000 VMs, with 50 running concurrently}
    \label{fig:boottime_chart_1000}
\end{figure}
\begin{table}[h]
    \centering
\csvreader[
  tabular=lrrrrrr,
  table head=\toprule {Type} & {p95} & {p95 Change} & {Std. Deviation} \\\midrule,
  late after last line=\\\bottomrule\newline
]{
  figure/boottime_table_1000.csv
}{}{\csvcoli & \csvcolv & \csvcolvi & \csvcolvii}
\caption[Boot Times for 1000 VMs]{Boot time for 1000 VMs, with 50 VMs running concurrently}
    \label{tab:boottime_table_1000}
\end{table}

\subsubsection*{Memory Overhead}
%The results showed no divergence when different VM memory sizes were used, verifying a stable overhead. 
%The change in memory overhead for the 3 setups can be seen in \autoref{tab:memoverhead_table}.
%When only the Firecracker process was measured, the difference was only $4$KB, corresponding to an $0.16$\% increase.
%However, when including the memory of the swtpm process, the impact was significantly greater showing an increase of a total of $52.35$\%.
%The significance of the $3760$KB overhead is further discussed in Section~\ref{disc_memoverhead}.
The results confirmed stable overhead across different VM memory sizes. 
Memory overhead for the three setups is presented in \autoref{tab:memoverhead_table}. 
Measuring only the Firecracker process indicated a minimal increase of $4$KB ($0.16$\%). 
However, when accounting for the swtpm process memory, the overhead increased by a total of $3760$KB ($52.35$\%). 
This is further discussed in Section~\ref{disc_memoverhead}.

\begin{table}[h]
    \centering
\csvreader[
  tabular=lrr,
  table head=\toprule  & KB Overhead & Change \\\midrule,
  late after last line=\\\bottomrule\newline
]{
  figure/memoverhead_table.csv
}{}{\csvlinetotablerow}
\caption[Memory Overhead Results]{Memory overhead of Firecracker and corresponding percentage increase}
    \label{tab:memoverhead_table}
\end{table}


\subsection{Attack Surface Analysis}
%As Firecracker aim to have a minimal implementation, there is relevancy in understanding what impact the modifications have.
%The modified Firecracker VMM compared to the original code in terms of the number of lines of code, was examined using the command line program CLOC~\cite{aldanial_cloc_2022}. 
%Considering only program code, disregarding configuration files, there was only an increase of approximately $2$\% lines of code (which corresponds to an addition of 1257 lines for a total of 61 697).
Analysed using CLOC~\cite{aldanial_cloc_2022}, the modified Firecracker VMM added approximately $2$\% more lines of code compared to the original code (adding 1257 lines to a total of 61 697), resulting in a minimal increase.

The communication between a guest and the hypervisor code had no change in the attack surface, considering Firecracker already handles virtio support.
%Instead, we made a comparison between the network device and the TPM device, regarding their communication between the hypervisor internals and the host OS.
%The virtual network device creates a simulated network device using a call to a Linux kernel module that executes code based on the configuration supplied to Firecracker.
%Therefore, all network calls in the guest will pass through the kernel. 
%This procedure can be compared with the TPM device in Firecracker that communicates with swtpm -- a userspace process on the host --, therefore being significantly less privileged. 
Instead, comparing communication between the hypervisor internals and the host OS for both the network device and the TPM device, we observed that network calls pass through the kernel, while the TPM device communication with swtpm -- a userspace process on the host -- which has lower privilege levels and less potential for exploitation.

%Seeing that the vTPM device in Firecracker passes the data from the guest to the swtpm process itself, it should be considered an extension of the attack surface. 
%Swtpm, implemented in C, poses a potential target for adversaries due to memory safety issues, as can be seen in recent issues~\cite{falcon_vulnerabilities_2023}.
%Such issues can lead to code execution vulnerabilities, which in the case of an swtpm process interfaced from a Firecracker VM, implies a VM escape. 
%However, since the swtpm process runs in the host userspace, defence-in-depth principles can be used to isolate the process from the rest of the system. 
Data passed from the guest to swtpm is an extension of the attack surface. 
Swtpm, running in the host userspace and implemented in C, has recently experienced issues~\cite{falcon_vulnerabilities_2023}. However, applying defense-in-depth principles can isolate it from the system. 
%
%These findings clearly indicated that the greatest change in the attack surface originates from the swtpm program itself and not from the integrated TPM functionality in Firecracker.
The primary change in the attack surface came from swtpm itself and not from the integrated TPM functionality in Firecracker.

==> content_new/design_implementation.tex <==
\section{Design and Implementation}\label{des_impl}
In this section, we introduce the changes made to Firecracker to support a vTPM.

\subsection{High-level Description}
%The current virtual device capabilities of Firecracker are small, focusing on devices adhering to the virtio standard~\cite{russell_virtio_2008}.
%The TPM is usually discovered using \textit{Advanced Configuration and Power Interface} (ACPI), but to fit the current Firecracker device model that does not support ACPI, the virtual device implemented in this project uses virtio.
%After analysing different VMMs, only crosvm~\cite{crosvm_2023} uses TPM over virtio, in comparison to QEMU and Cloud-Hypervisor, which both use ACPI~\cite{bellard_qemu_2005,cloud-hypervisor}.
Firecracker's virtual device capabilities are small, adhering to the virtio standard~\cite{russell_virtio_2008}. 
To enable vTPM support without \textit{Advanced Configuration and Power Interface} (ACPI), we employ virtio. 
Crosvm~\cite{crosvm_2023} is the only VMM using TPM over virtio, unlike QEMU and Cloud-Hypervisor, which both use ACPI~\cite{bellard_qemu_2005,cloud-hypervisor}. 
%
%The updated Firecracker device model can be seen in \autoref{fig:tpm-additions}. 
%The boxes with blue, dotted outlines denote the added components from open-source projects, whereas the boxes with green, dashed outlines are the components implemented in this project. 
%The boxes inside the Firecracker box represent device interfaces between the host and the guest.
%The specific vTPM implementation on the host used in this project is swtpm~\cite{vtpm}.
%The virtio-tpm device driver on the guest side uses the already existing architecture for TPMs in the Linux kernel and integrates with the IMA~\cite{tolnay_chromium_nodate}.
Our updated Firecracker device model, seen in \autoref{fig:tpm-additions}, includes components from open-source projects (blue, dotted outlines) and those implemented in this project (green, dashed outlines). 
The boxes inside the Firecracker box represent device interfaces between the host and the guest.
Our vTPM implementation uses swtpm~\cite{vtpm} on the host and integrates existing architecture for TPMs in the Linux kernel and integrates with the IMA~\cite{tolnay_chromium_nodate}.

%To run a Firecracker VM with a TPM, some cryptographic certificates and keys need to be created to associate the vTPM with the hardware TPM on the host. 
%After that, the vTPM should be started with a file path passed to it. 
%The vTPM will then create a communication socket on that file path. 
%This socket then needs to be passed to the Firecracker VM configuration, along with a Linux kernel compiled with virtio-tpm support.
%Then the Firecracker VM can be started and will have access to the vTPM.
To run a Firecracker VM with a TPM, create cryptographic certificates to associate the vTPM with the host's hardware TPM, start the vTPM with a file path.
Then, pass the communication socket created on that file path, to the Firecracker VM configuration, along with a Linux kernel compiled with virtio-tpm support.
Then the Firecracker VM can be started with access to the vTPM.

\begin{figure}[h]
    \centering
    \includegraphics[width=80mm]{figure/fc-tpm.png}
    \caption[Firecracker Device Model with TPM Support]{The device model of Firecracker with TPM device support}
    \label{fig:tpm-additions}
\end{figure}

\subsection{Technical Implementation}
The implementation of the TPM device in Firecracker can be seen in \autoref{fig:firecracker-tpm-class-changes}. 
%The two main components can also be seen in \autoref{fig:tpm-additions} as the two green arrows.
%\emph{SWTPMBackend} is the arrow from the vTPM to the TPM and \emph{TPMVirtioDevice} can be seen as the arrow between the TPM box and the virtio-tpm box.
The two main components, \emph{SWTPMBackend} and \emph{TPMVirtioDevice}, also seen as the green arrows in \autoref{fig:tpm-additions}, connect the vTPM, TPM, and virtio-tpm device driver. 

\begin{figure}[h]
    \centering
    \includegraphics[width=80mm]{figure/fctpm_UML.png}
    \caption[Class Diagram of Firecracker Changes]{An UML class diagram, the green boxes with dashed borders are added implementations to Firecracker}
    \label{fig:firecracker-tpm-class-changes}
\end{figure}


Inspired by the Cloud-Hypervisor project~\cite{cloud_hypervisor_2023}, \emph{SWTPMBackend}, the arrow from the vTPM to the TPM, uses swtpm over a UNIX socket.
%The \emph{SWTPMBackend} was inspired by the vTPM implementation in the Cloud-Hypervisor project~\cite{cloud_hypervisor_2023}, as they also use swtpm over a UNIX socket.
To account for platform setup procedures, swtpm exposes a control channel, which is used to both initialise the TPM and to set a file descriptor for client TPM commands.
The file descriptor is one side of another UNIX socket that is created in \emph{SWTPMBackend}. 
The other side of that socket is used to send and receive messages inside Firecracker. 

\emph{TPMVirtioDevice}, the arrow between the TPM box and the virtio-tpm box, implements the \emph{MutEventSubscriber} and \emph{VirtioDevice} utilizing existing interfaces in Firecracker for device discovery and management. 
%The \emph{TPMVirtioDevice} implements the \emph{MutEventSubscriber} and \emph{VirtioDevice} interfaces which already exists in Firecracker.
%By using these interfaces, the virtual device fits into the Firecracker device model, and no major changes were needed regarding the internals of Firecracker. 
%Another major advantage of implementing these interfaces was that interrupt registration and device activation are taken care of by already existing components within Firecracker.
Firecracker also passes the memory address of the device automatically to the kernel command line parameters for device discovery by the Linux kernel.

%In the virtual device implementation, a single queue is used for communication between the VM and Firecracker. 
%Using a single queue was possible as it is always the client who initiates communication in the case of a TPM, which can be compared with a network device where any side might initiate communication. 
%This difference is also apparent when comparing the virtio network device in Firecracker with our virtio TPM device, as the virtio network device uses two queues. 
Communication between the VM and Firecracker takes place through a single queue since the TPM client always initiates communication. 
This differs from the network device in Firecracker, where either side can initiate communication, requiring two queues.


%The source code for the virtual TPM device, as well as the resources required to reproduce the benchmarks described in the next section, can be found in a GitHub37RECYR1 repository~\footnote{\url{https://github.com/DATX05-CSN-8/fctpm-2023/tree/paper}}.
The virtual TPM device source code and benchmark resources are available on GitHub repository~\footnote{\url{https://github.com/DATX05-CSN-8/fctpm-2023/tree/paper}}.

==> content_new/discussion.tex <==
\section{Discussion}\label{discussion}
%This section discusses the results of the experiments, measurements, and analyses performed, with respect to both performance and security. 
%The impact on performance and security introduced by adding TPM support to Firecracker is evaluated in a real-world scenario with CSPs in mind. 
%Additionally, limitations and potential measurement errors are discussed. 
This section discusses the results of our experiments, focusing on performance and security implications. 
We evaluate the impact of adding TPM support to Firecracker in a real-world CSP scenario and discuss limitations and potential measurement errors.

\subsection{Performance Evaluation}
%In this section we first discuss various aspects regarding the startup time and then the results of the memory overheads.
In this section, we examine startup time and memory overheads.

\subsubsection{Startup Time Evaluation}
%The results for the concurrent test scenario using the pooled setup showed an $17$\% increase which might seem quite major. 
%However, since the usage of a TPM in PaaS solutions would be an opt-in feature, similar to that of the current IaaS, customers will have the flexibility to choose whether or not to utilize this functionality.
%Additionally, the CSP could charge an additional fee for this functionality, depending on whether the performance impact hits the CSP or the customer. 
We observed a $17$\% increase in startup time for the concurrent test scenario with the pooled setup. 
However, since TPM usage in PaaS is optional similar to current IaaS, customers can choose whether to use it, possibly incurring an additional fee. 
%
%Furthermore, since the output of the Firecracker internal boot timer device was compared with the values measured by the test suite, measurement errors can be ignored. 
%The startup time saw quite a major increase regarding the pooled setup moving Scenario 1 to Scenario 2. 
%As measurement errors were ruled out by comparing with the internal boot timer, we can consider the communication introduced between the Firecracker hypervisor and the vTPM as a root cause. 
Furthermore, as Firecracker internal boot timer device was compared with the values measured by the test suite, measurement errors were ruled out.  
The communication between the Firecracker hypervisor and vTPM was instead identified as a key factor for the increase.

%The virtual TPM device implemented in Firecracker is synchronous, meaning that the hypervisor wakes up as the guest notifies the device, after that the request is sent to the vTPM, and the guest stays paused for the time it takes to process the request.
%Also, when sending and receiving data from the SWTPMBackend, the Firecracker process is blocked due to IO calls to the file descriptor communicating with the swtpm process. 
%The IO calls cause the process to go to sleep; meanwhile, another process might start to execute, which can cause a delay. 
%As the number of concurrent processes increases, the risk that the Firecracker process needs to wait before executing again after a blocking call increases. 
The virtual TPM device in Firecracker operates synchronously, causing the guest to pause while processing requests. 
Also, sending and receiving data from SWTPMBackend, the IO calls to the file descriptor communicating with the swtpm process block the Firecracker process, potentially leading to delays. 

%When comparing the startup time results in this project with the values in the Firecracker research paper~\cite{firecracker-paper}, the difference is significant. 
%A reason behind the difference in startup time is the different hardware setups used, mainly the CPU used could have impacted the result. 
%The CPU used by \textcite{firecracker-paper} is more performant in comparison to the one used in this project. 
%Both single-thread performance and multi-thread performance are significantly lower in this project compared to the one used in the Firecracker research paper. 
%Important for the concurrent scenario is the number of cores, which in the Firecracker paper totalled 48, compared to the 32 used in this project. 
%An important aspect regarding the number of cores is the difference between the total number of cores and the desired parallelism. 
%Logically, as the number of cores is lower in comparison with the desired parallelism, the host OS needs to make vital scheduling decisions.
%These decisions may have caused some workloads to wait, which might have been a reason for the performance difference.
The significant difference compared to Firecracker's research paper~\cite{firecracker-paper}, results from distinct hardware setups, mainly the CPU used.
The CPU in \textcite{firecracker-paper} is more performant in comparison to the one used in this project. 
Single-thread and multi-thread performance in this project are significantly lower than in the Firecracker research paper. 
The Firecracker paper used 48 cores, while this project used 32. 
The disparity between the total core count and desired parallelism necessitates crucial scheduling decisions by the host OS, potentially causing workloads to wait, contributing to the performance gap.

%Regarding the usage of a resource pool, considering real-world use, there would not be a situation where a CSP would allocate vTPMs on demand. 
%Cloud providers go to great lengths to minimise the critical execution path to improve the response times of their PaaS offerings.
%Therefore, if there is an option to use a resource pool, CSPs have no reason not to use it.
%However, the pool algorithm featured in this work is not suitable for real-world PaaS environments, as it assumes that the total number of virtual machines is known in advance. 
In real-world scenarios, CSPs would not allocate vTPMs on demand. 
Therefore, if there is an option to use a resource pool, CSPs would likely use it.
However, the pool algorithm proposed in this study assumes advance knowledge of VM numbers, making it unsuitable for typical PaaS environments.

\subsubsection{Memory Overhead Evaluation}
\label{disc_memoverhead}
%With regards to the memory overhead comparing the unmodified Firecracker and Firecracker with TPM support, a static increase of 4KB was observed regardless of the VM memory size. 
%Such an increase is minor and would be considered tolerable by a CSP. 
%However, including the overhead of the swtpm process, the total overhead amounts to 3760KB.
%Which, considering the total memory allocation of a VM still corresponds to a minor part of the total memory allocated, typically a minimum of 128MB. 
Regarding memory overhead, Firecracker with TPM support showed a static $4$KB increase regardless of VM memory size, a minor increase, tolerable by a CSP.
When including swtpm process overhead, the total amounts to $3760$KB, still a small fraction of a typical VM allocation, typically a minimum of $128$MB.

%Another aspect is to compare Firecracker to QEMU and Cloud-Hypervisor.
%\textcite{firecracker-paper} stated that Firecracker have the smallest overhead at approximately 3MB, whereas Cloud-Hypervisor came second at approximately 13MB, and QEMU last at 131MB~\cite{firecracker-paper}. 
%Considering the overhead of the other hypervisors, the increase seen when adding TPM support is negligible. 
Comparing Firecracker to QEMU and Cloud-Hypervisor, Firecracker had the smallest overhead at around $3$MB, followed by Cloud-Hypervisor at approximately $13$MB, and QEMU with the highest at $131$MB~\cite{firecracker-paper}. 
Considering the overhead of other hypervisors, the increase with TPM support is negligible.

%As stated, the memory overhead of the resource pool was not considered during the tests.
%This is mainly due to the pooling algorithm used as it pre-allocates TPMs for the total number of VMs, which means it consumes more memory compared to a dynamically allocating algorithm. 
As stated, the memory overhead of the resource pool was not considered due to its pre-allocation algorithm, consuming more memory compared to dynamic allocation.

\subsection{Security Analysis}
\label{disc_security_evaluation}
The result of the attack surface analysis highlights that the major change in the attack surface is seen in the swtpm process.
As it is not an option to limit the communication with the swtpm process from the Firecracker hypervisor --considering it needs to adhere to the TPM specification --, other security hardening options have to be used.
Assuming the worst, that an adversary can achieve code execution through the TPM commands to the swtpm process, applying defence-in-depth principles come naturally to isolate the adversary and minimise the impact that can be made. 
Defence-in-depth can be applied and used in multiple ways; one alternative is to isolate the process using Linux kernel primitives, another is to run the vTPM in a separate VM as done with CoCoTPM~\cite{pecholt_cocotpm_2022}.

\subsubsection{Isolating with Linux Kernel Functionality}
To harden the security of the swtpm process, Linux cgroups, namespaces, and seccomp filters can be used, among others. 
Using cgroups can mitigate host resource exhaustion if the adversary floods the swtpm process through the TPM interface. 
Namespaces improve process isolation by exposing an abstracted view of the network, the process table, and the directory structure to the environment of the swtpm process. 
Therefore, the use of namespaces can mitigate potential pivots of an adversary, as it can limit the network capability of the process.
By using seccomp filters, the \textit{system calls} (syscalls) a process can perform are limited to a specific set. 
As the vTPM emulates a self-contained hardware component with limited connectivity, few syscalls need to be allowed by the seccomp filters, showcasing the applicability for this use case.

\subsubsection{Alternative Isolation Methods}
Another option to improve the security of the vTPM implementation is to contain the emulation within the Firecracker program itself. 
Containing the emulation within Firecracker would, however, increase the program size and memory use of the Firecracker process along with coupling the two components together, which might be undesirable for a CSP. 
Also, if the swtpm code were to be part of the Firecracker process, an arbitrary code execution exploit would achieve the privilege of the Firecracker process.
Therefore, an adversary would have more access compared to the case where swtpm is a separate, hardened process.

Containing the vTPM in a separate environment is another option, which would improve isolation even more, at the price of increased overhead. 
Previous work within the space shows both solutions in separate VMs as well as TEEs~\cite{pecholt_cocotpm_2022,svtpm_a_2019}.

Although the security impact can be interpreted as major due to the risk of vulnerabilities in the vTPM implementation, the time to patch a software component is significantly shorter compared to patching a hardware implementation or firmware. 
Combining the shortened patch time with the fact that CSPs already use vTPMs in their IaaS offerings implies that the security impact is considered acceptable. 


==> content_new/intro.tex <==
\section{Introduction}


Cloud computing has transformed the way we store, access, and process data.
%The ability to access and use computing resources on demand, without the need for large upfront investments in hardware and infrastructure, has made cloud computing an attractive and flexible option for businesses of all sizes~\cite{surbiryala2019cloud}.
%Cloud computing has revolutionised data storage, access, and processing. 
The flexibility to access computing resources on demand, without upfront investments in hardware and infrastructure, makes it an attractive and flexible option for businesses~\cite{surbiryala2019cloud}.

By transferring on-site infrastructure to cloud computing platforms, more control and trust is given to the third-party company hosting the service. 
In practice, companies let cloud providers execute their software and process potentially sensitive data of their customers. 
To secure both the system running and the handling of data, safe storage and verification of the platform should be implemented to ensure trust properties.

%One way to achieve trust in a computer system is to use a \textit{Trusted Platform Module} (TPM), which is a coprocessor for secure cryptographic support. 
%Considering cloud infrastructure, the customer is most often given a \textit{virtual machine} (VM), which can be equipped with a \textit{virtual TPM} (vTPM). 
%This vTPM is also considered trusted, as there are multiple ways to associate such a TPM with trusted hardware~\cite{vtpm}.
%However, in the case where cloud providers maintain both the machine as well as the operating system, there is no one who exposes trusted computing functionality such as a TPM.
One way to achieve trust in a computer system is to use a \textit{Trusted Platform Module} (TPM), a coprocessor for secure cryptographic support. 
Trusted Platform Module (TPM) is essential for system trust. 
Cloud customers are often provided with a \textit{virtual machine} (VM) which can be equipped with a virtual TPM (vTPM)~\cite{vtpm}. 
However, in the case where cloud providers maintain both the machine as well as the operating system, trusted computing functionality is absent.


%Virtual machines driven by the Firecracker~\cite{firecracker-paper} \textit{Virtual Machine Monitor} (VMM), also called hypervisor in this paper, do not offer TPM device functionality.
%Yet, Firecracker is used in offerings by \textit{Amazon Web Services} (AWS), the main cloud provider in the world as of today~\cite{zhang_top_2023}.
%Firecracker was created with the goals of workload isolation, low startup times, and low memory overhead. 
%To achieve minimal overhead, several trade-offs have been made compared to traditional VMMs. 
%Typically, there is only support for a minimal device model, therefore not including TPM device support.
%As a result, incorporating a TPM in such an environment might have an impact on said performance properties, such as memory overhead and startup times.
Virtual machines powered by Firecracker~\cite{firecracker-paper} \textit{Virtual Machine Monitor} (VMM), also called hypervisor in this paper, lack TPM support. 
Yet, Firecracker is used in offerings by \textit{Amazon Web Services} (AWS), the main cloud provider in the world as of today~\cite{zhang_top_2023}.
Firecracker was designed to focus on workload isolation, low startup times and low memory overhead. 
Integrating TPM support into Firecracker's minimal device model could potentially impact these performance aspects, including memory overhead and startup times.
Increased communication between the VM and hypervisor internals could compromise workload isolation due to an expanded attack surface.

%By extending the Firecracker device model, the communication between the VM and hypervisor internals is also increased. 
%Such a modification can have an impact on the attack surface, which would deteriorate workload isolation.

%In order to tackle the challenges aforementioned, we address in this paper the following research questions:
This paper addresses three research questions:
\begin{enumerate}
  %\item How does the startup time and memory overhead of a Firecracker VM change if a vTPM is created and allocated to it?
  %\item What impact on the startup time does maintaining a resource pool of TPMs to be allocated have?
  \item How does vTPM allocation impact Firecracker VM startup time and memory overhead?
  \item What is the impact of maintaining a TPM resource pool on startup time?  
  \item How does incorporating a TPM change the attack surface of a lightweight VM?
\end{enumerate}

%It is important to note that while this paper does not present a complete solution for TPMs in \textit{platform-as-a-service} (PaaS) offerings, it serves as a crucial building block towards the development of a trusted PaaS environment. 
%Trusted computing already exists within \textit{infrastructure-as-a-service} (IaaS) frameworks which this paper builds upon to contribute to the field through the following key aspects:
While this paper does not present a complete solution for TPMs in \textit{platform-as-a-service} (PaaS) offerings, it serves as a crucial building block towards the development of a trusted PaaS environment. 
This work builds upon existing trusted computing frameworks in \textit{infrastructure-as-a-service} (IaaS), focussing on:

\begin{itemize}
\item Introducing TPM device support in Firecracker, ensuring the compatibility and goals of Firecracker.
\item Addressing resource pooling requirements for TPMs in PaaS environments, to act as a base for future efficient and scalable implementations.
\item Conducting a comprehensive security analysis of vTPM usage, highlighting the strengths and potential vulnerabilities associated with its implementation.
\end{itemize}
By focusing on these specific contributions, our research aims to provide valuable insights and advancements towards trusted PaaS offerings, promoting secure and reliable cloud computing platforms.

%The rest of this paper is organised as follows. 
%Section~\ref{related_work} reviews related concepts whilst Section~\ref{des_impl} describes how the TPM support is integrated into Firecracker.
%Section~\ref{bench_resul} describes the design of the test suite and then presents the results of the performance tests and attack surface analysis.
%In Section~\ref{discussion}, the results and possible impacts are discussed, and finally, Section~\ref{conclusion} concludes the paper.
The rest of this paper is organised as follows. 
Section~\ref{related_work} reviews related concepts whilst Section~\ref{des_impl} describes TPM integration into Firecracker.
Section~\ref{bench_resul} covers the test suite design and presents performance test results and the attack surface analysis.
Section~\ref{discussion} discusses the results and possible impacts, and finally, Section~\ref{conclusion} concludes the paper.


==> content_new/related_work.tex <==
\section{Related Work}\label{related_work}
%This chapter is dedicated to explaining the current state-of-the-art in the space of trusted cloud computing and virtualisation technologies within Paas offerings. 
This chapter provides an overview of the current state of trusted cloud computing and virtualisation technologies in PaaS offerings.



\subsection{VTPM Implementation Models}
%To improve performance, avoid data leakage and isolation issues in vTPMs, \textcite{svtpm_a_2019} continued the work of \textcite{vtpm} and created an alternative TPM software implementation, called \textit{Secure vTPM} (SvTPM).  
%The novelty of their work is to base the trust in a TEE instead of a hardware TPM. 
%More specifically, they use Intel SGX to run or protect specific parts of the TPM in an SGX enclave.  
%Their work resulted in a much lower startup time in comparison to previous implementations.
%Similarly, but more cross-platform adapted, initiatives such as HyperEnclave~\cite{jia_hyperenclave_2022} use the integrity measurement and attestation capabilities of a TPM to extend the chain of trust to the TEE.
To improve vTPM performance, address data leakage and isolation issues, \textcite{svtpm_a_2019} continued the work of \textcite{vtpm} and introduced \textit{Secure vTPM} (SvTPM), relying on Intel SGX for trust in a TEE instead of a hardware TPM. 
This approach significantly reduces startup time. 
Initiatives like HyperEnclave~\cite{jia_hyperenclave_2022} also extend trust using TPM attestation capabilities.
Similarly, but more cross-platform adapted, initiatives such as HyperEnclave~\cite{jia_hyperenclave_2022} also extend the chain of trust to the TEE using TPM attestation capabilities.

%Another approach to achieve similar goals is called \textit{Confidential Computing TPM} (CoCoTPM).
%CoCoTPM minimises the trust required towards the host and the hypervisor by running a vTPM in an encrypted VM using AMD SEV.
%The communication between these TPMs and the other VMs running the desired workload is encrypted and integrity protected, further increasing the confidentiality property~\cite{pecholt_cocotpm_2022}.
Another approach is \textit{Confidential Computing TPM} (CoCoTPM), running a vTPM in an encrypted VM using AMD SEV to minimise the trust required towards the host which enhance confidentiality~\cite{pecholt_cocotpm_2022}.
%
%However, to keep our contributions applicable to practical usecases, \textit{swtpm}~\cite{vtpm} is used in the experiments of this work. 
%Swtpm is used by hypervisors such as QEMU and Xen.
However, for practical purposes, this work employs \textit{swtpm}~\cite{vtpm}, used by hypervisors like QEMU and Xen.

\subsection{Trust in Cloud Computing Environments}
%In a literature study on trust in cloud computing, \textcite{AMIbrahim2019} highlight the significant role of the TPM.
%They investigate different architectures and managers for IaaS services, compare different vTPMs and remote attestation types, and discuss secure boot and integrity monitoring. 
In a literature review of trust in cloud computing, \textcite{AMIbrahim2019} emphasize the role of the TPM, exploring various IaaS architectures, vTPMs, remote attestation, secure boot, and integrity monitoring.

%Considering PaaS offerings, \textit{Cloud Service Providers} (CSPs) are required to make a decision whether to use containerisation or virtualisation.
%This comparison has seen a lot of research, both on performance and isolation~\cite{felter_updated_2015,chae_performance_2019,tesfatsion_virtualization_2018,morabito_hypervisors_2015}.
Regarding PaaS, \textit{Cloud Service Providers} (CSPs) must decide between containerisation and virtualisation, an extensively researched topic~\cite{felter_updated_2015,chae_performance_2019,tesfatsion_virtualization_2018,morabito_hypervisors_2015}.
%
%Recent development within the space of runtimes for PaaS offerings has been seen with Google gVisor from the container side, and AWS Firecracker from the virtualisation side. 
%\textcite{young2019true} conducted a study comparing the gVisor runtime and the default Docker runtime.
%Their results show a significant decrease in performance with respect to system calls, memory allocations, and networking. 
%Another comparison between Firecracker and gVisor made by \textcite{anjali_blending_2020}, resulted in favour of Firecracker for network bandwidth, memory allocation times, and file access.
Recent developments within the space of runtimes for PaaS offerings include Google gVisor for containers and AWS Firecracker for virtualization. 
Performance comparisons favor Firecracker in terms of network bandwidth, memory allocation times, and file access~\cite{young2019true,anjali_blending_2020}.

%If we consider trusted computing in PaaS offerings, efforts on integrity-verified containers can be applied to solutions such as gVisor. 
%An example of such work is Container-IMA by \textcite{luo2019container}.
%The attestation mechanism they propose improves privacy of the container and the underlying host and ensures container isolation.
%Instead of including support for vTPMs in user space, the mechanism uses a shared measurement agent in kernel space, where all application layers are measured by the IMA.
%The novelty of their work lies in their method for multiplexing PCRs for ephemeral container workloads.
Integrity-verified containers, such as Container-IMA~\cite{luo2019container}, enhance privacy and isolation in PaaS offerings. 
It uses a shared kernel-based measurement agent, multiplexing PCRs for transient container workloads.
Instead of implementing vTPM support in user space, it utilises a shared kernel-based measurement agent that assesses all application layers using IMA. 
The novelty of their work lies in their method for multiplexing PCRs for ephemeral container workloads.
%
%However, for PaaS solutions based on virtualisation, such as Firecracker, no effort has been made to enable trusted or confidential computing.
%As our work aims to integrate TPMs into Firecracker, other components are needed to provide trust, confidentiality, and integrity to PaaS offerings.
%Already available components, such as the mentioned SvTPM~\cite{svtpm_a_2019} and Linux IMA~\cite{sailer_ima_2004} can be used alongside our contributions to build a complete system. 
However, for virtualization-based PaaS such as Firecracker, no prior effort exists for trusted or confidential computing. 
Our work aims to integrate TPMs into Firecracker, which can be combined with existing components like SvTPM~\cite{svtpm_a_2019} and Linux IMA~\cite{sailer_ima_2004} to create a comprehensive system.
